Detailed Decomposition of Galaxy Images. II. Beyond Axisymmetric Models

We present a two-dimensional (2-D) fitting algorithm (GALFIT, Version 3) with new capabilities to study the structural components of galaxies and other astronomical objects in digital images. Our technique improves on previous 2-D fitting algorithms by allowing for irregular, curved, logarithmic and power-law spirals, ring and truncated shapes in otherwise traditional parametric functions like the Sersic, Moffat, King, Ferrer, etc., profiles. One can mix and match these new shape features freely, with or without constraints, apply them to an arbitrary number of model components and of numerous profile types, so as to produce realistic-looking galaxy model images. Yet, despite the potential for extreme complexity, the meaning of the key parameters like the Sersic index, effective radius or luminosity remain intuitive and essentially unchanged. The new features have an interesting potential for use to quantify the degree of asymmetry of galaxies, to quantify low surface brightness tidal features beneath and beyond luminous galaxies, to allow more realistic decompositions of galaxy subcomponents in the presence of strong rings and spiral arms, and to enable ways to gauge the uncertainties when decomposing galaxy subcomponents. We illustrate these new features by way of several case studies that display various levels of complexity.

==> table-header.tex <==
\begin{deluxetable*}{|c|c|r|rrrrrrr|l|}
\tabletypesize{\scriptsize}
\tablewidth{0pt}
\tablecaption {M51 Fitting Results}
\tablehead{  
  & \#  & --- sersic --- & $\Delta x$ [\arcsec] & $\Delta y$ [\arcsec] &  mag    &   $r_e$ [\arcsec]  &   $n$     &  $q$      &  $\theta_{\rm{PA}}$ [deg]   & Comments \\ 
  & \#  & --- sersic3 --- & $\Delta x$ [\arcsec] & $\Delta y$ [\arcsec] &  mag/\arcsec$^2$  &   $r_e$ [\arcsec]  &   $n$     &  $q$      &  $\theta_{\rm{PA}}$ [deg]   & Comments \\ 
  &     & power &    ---      &    $R_{\rm{bar}}$ [\arcsec]&  $R_{\rm{out}}$ [\arcsec] &  $\theta_{\rm{rot}}$ [deg] & $\alpha$   &  $\theta_{\rm{incl}}$ [deg] &  $\theta_{\rm{sky}}$ [deg]& \\ 
  &     & four &    ---      & \multicolumn{2}{r}{mode: ampl. \& phase [deg]} & \multicolumn{2}{r}{mode: ampl. \& phase [deg]}  & \multicolumn{2}{r|}{mode: ampl. \& phase [deg]} & \\
  &     & bend &    ---      & \multicolumn{2}{r}{mode: amplitude [\arcsec]} & \multicolumn{2}{r}{mode: amplitude [\arcsec]}  & \multicolumn{2}{r|}{mode: amplitude [\arcsec]} & \\
  & \#  & sky  & $\Delta x$  & $\Delta y$  &  $c$    &  $dc/dx$  &  $dc/dy$  & --- & --- & }
\startdata
\enddata
\tablecomments{See Table~\ref{arp147-table} for details.}
\label{m51tab}
\end{deluxetable*}

